Improved Calibration of Numerical Integration Error in Sigma-Point Filters

The sigma-point filters, such as the UKF, which exploit numerical quadrature to obtain an additional order of accuracy in the moment transformation step, are popular alternatives to the ubiquitous EKF. The classical quadrature rules used in the sigma-point filters are motivated via polynomial approximation of the integrand, however in the applied context these assumptions cannot always be justified. As a result, quadrature error can introduce bias into estimated moments, for which there is no compensatory mechanism in the classical sigma-point filters. This can lead in turn to estimates and predictions that are poorly calibrated. In this article, we investigate the Bayes-Sard quadrature method in the context of sigma-point filters, which enables uncertainty due to quadrature error to be formalised within a probabilistic model. Our first contribution is to derive the well-known classical quadratures as special cases of the Bayes-Sard quadrature method. Then a general-purpose moment transform is developed and utilised in the design of novel sigma-point filters, so that uncertainty due to quadrature error is explicitly quantified. Numerical experiments on a challenging tracking example with misspecified initial conditions show that the additional uncertainty quantification built into our method leads to better-calibrated state estimates with improved RMSE.

==> tab/ungm_nll.tex <==
\begin{table}[!h]
	\centering
	\smallskip
	\begin{tabular}{@{} l S[table-format=2.8] S[table-format=1.8] S[table-format=1.6] @{}}
		\toprule
		\text{Point-set} 	& \text{Classical} 	& \text{Bayes--Sard}	& \text{GPQ} 		\\
		\midrule
		UT   				& 28.027 \pm 0.993 	& 4.144 \pm 0.029 	& 4.025 \pm 0.025 	\\
		GH-5 				& 20.537 \pm 0.905 	& 3.648 \pm 0.012 	& 3.739 \pm 0.009 	\\
		GH-7 				& 16.882 \pm 0.711 	& 3.621 \pm 0.013 	& 4.145 \pm 0.011 	\\
		\bottomrule
	\end{tabular}
	\caption{The average NLL on UNGM example with bootstrapped 2 standard deviations (in parentheses).}
	\label{tab:unmg_nll}
\end{table}

